Scheduling Network Function Chains Under Sub-Millisecond Latency SLOs

Network Function Virtualization (NFV) seeks to replace hardware middleboxes with software-based Network Functions (NFs). NFV systems are seeing greater deployment in the cloud and at the edge. However, especially at the edge, there is a mismatch between the traditional focus on NFV throughput and the need to meet very low latency SLOs, as edge services inherently require low latency. Moreover, cloud-based NFV systems need to achieve such low latency while minimizing CPU core usage. We find that real-world traffic exhibits burstiness that causes latency spikes of up to 10s of milliseconds in existing NFV systems. To address this, we built NetBlaze, which achieves sub-millisecond p99 latency SLOs, even for adversarial traffic, using a novel multi-scale core-scaling strategy. NetBlaze makes traffic-to-core allocation decisions at rack, server, and core-spatial scales, and at increasingly finer timescales, to accommodate multi-timescale bursts. In comparison with state-of-the-art approaches, NetBlaze is the only one capable of achieving sub-millisecond p99 latency SLOs while using a comparable number of cores.

==> design.tex <==

% Flow-level load balancing is not practical for realistic traffic
% why not practical? then what's the solution?

\section{System Design}
\label{sec:design}

% 0) system overview and components:
% - NFVCtrl, NFVCore & NFVRCore, NFVMonitor (for generating NF profiles)
% Need to mention: why these components are new and critical for our design

We first provide a high-level overview of \sysname, and discuss a list of system components. We then summarize the key idea and clarify our critical design choices.


\subsection{System overview}
\label{subsec:system-overview}

\sysname is a controller that works for a cluster of servers, running NFV chains that consist of one or many NFs. \sysname's key feature is to allow users to associate each chain with a target tail latency SLO. It then adapts to traffic dynamics to meet the target while achieving good CPU core efficiency.


To schedule an NF chain with \sysname, users need to provide an \textit{NF chain specification} which includes a description of NFs that \sysname should run and the way of forming a packet processing pipeline with these NFs.



\subsection{System components}
\label{subsec:system-components}

\parab{NFV controller.} This per-worker controller manages the dispatching of incoming packets and the execution of NF chains on a multi-core server. It does so by interacting with other system components, i.e. NICs, normal CPU cores and reserved CPU cores. Upon initialization, the controller configures per-server NICs, and creates a pool of software queues, bringing up a pool of threads, each for running one or more NFs. By default, these NF threads are idle and not scheduled to run on CPU cores. At runtime, the controller is responsible to dispatch incoming packets, dispatch them into a number of software queues, assign each software queue to be handled by one NF thread, and then notify the per-core thread scheduler to start running / stop running NF threads to scale up/down. The controller is critical for scaling NF chains to meet the user specified tail latency SLO while keeping active CPU cores as busy as possible for a high efficiency.

\parab{Normal core.} In \sysname, each normal core (called NCore) is assigned with one NIC queue and one software queue. A normal core is responsible for 1) (periodically) pulling packet arrivals from the NIC queue designated to it and moving these packets to a number of software queues (w/ its own software queue preferred in this process); 2) running an NF thread, which does all required packet processing.

\parab{Reserved core.} In \sysname, each server maintains a number of reserved CPU cores (called RCore). These reserved cores are not assigned with NIC queues. Instead, they are assigned with on-demand software queues, which are borrowed by normal cores to absorb transient packet bursts. After being assigned with a software queue by NFVCtrl and woken up by the thread scheduler, each RCore starts by pulling packets from the queue, and runs the NF pipeline to process packets in batches.

\parab{NFV monitor.} The NFV monitor is a system component that helps produce a NF chain's profile in the offline profiling process. When in profiling mode, \sysname appends a NFV monitor module to each NF thread (running on its dedicated core). The NFV monitor module starts by turning on the NIC's hardware timestamp feature, and computes each packet's delay (i.e. the time spent on the server, beginning from the time arriving at the NIC's RX queue to the time leaving the NIC's TX queue). More details on generating an NF chain's performance profile are discussed later in the paper.

\subsection{Traffic assignment granularity}
% why are we doing this:
% two different granularity of traffic assignment?

% what is the system deployment scenario
In following sections, we discuss the set of design choices in \sysname within a basic scheduling unit, i.e. a rack-scale cluster of servers with one ToR. The ToR is the traffic ingress/egress of the cluster: incoming traffic arrives on a set of switch ports, while servers are also connected to the switch.

% high-flow rate makes it impossible to do per-flow routing at ToR
% software approach also suffers from the high latency
As a cluster scheduler, \sysname's task is to make traffic assignment decisions for incoming traffic, which consists of traffic flows (L3, L4 or L7). In general, most stateful NFs work on per-flow states, which requires \sysname to respect the flow-affinity constraint. For stateful NF chains, the smallest load balancing unit is a single flow. Prior work has proposed solutions that schedule individual flows \cite{wang2021galleon}. However, given a significantly large flow rate (i.e. more than $10k$ flow arrivals per second), we found that it is impossible to install a flow entry (at the ToR) for every new flow arrival.

% coarse-grained routing is bad for latency
On the other side, a different thread of prior work ~\cite{sosp15-e2,nsdi18-metron,conext19-rsspp} proposes to utilize hardware to group flows (either via hardware hash function or via hardware flow table) at the switch and NIC hardware to split traffic into traffic classes or RSS buckets. The traffic assignment granularity is larger than the per-flow basis. However, this approach is affected by both types of traffic burstiness in \secref{sec:motivation}. We've shown that NFV systems are not able to meet tail (\pnintynine) latency SLO if they are affected by transient bursts in incoming traffic.

% we propose a combined hierarchical routing:
% coarse-grained at ToR and NIC; fine-grained at normal cores;
We posit that an NFV system must employ a fine-grained per-flow assignment working at a microsecond-level time scale in order to handle transient traffic bursts. Given our observations on the high flow rate and frequent transient bursts in realistic traffic, we propose a hierarchical solution that employs a hybrid traffic assignment mechanism: at the hardware (ToR and NICs), \sysname utilizes the hardware-aided hash-based flow grouping to split incoming traffic into many groups of flows, while each group finally arrives at a server's NIC queue, and is uniquely pulled and processed by one normal CPU core. For each normal CPU core, it also employs a software-based flow-level traffic assignment mechanism that detects transient bursts, and pin-points culprit flows. Once a burst happens, this software-based fine-grained assignment approach can borrow software queues from NFVCtrl, which then triggers the execution of NF threads on the set of reserved cores at a server. In this way, incoming traffic is split across the cluster, while transient bursts can be handled, without violating the flow-affinity constraint.


% 1) the fine-grained admission control to absorb transient bursts with reserved cores
\input{op_short}

% 2) the coarse-grained admission control to pack RSS-buckets into normal cores
\input{op_long}

% 3) the actual profiling approach
\subsection{Profiling: the approach and details}

From experimentation, it is observed that the latency seen by a given network chain depends on two parameters, flow count and the packet rate. There are other parameters like CPU frequency and cache size that can impact the latency but these parameters are fixed and hence not considered. The offline profiler uses an artificial traffic generator to capture the relation between the packet rate and latency given the flow count and the network function chain. It uses a modified binary search algorithm to search for the paket rate threshold. The algorithm is biased towards lower packet rate as it double checks a packet rate, which does not exceed the threshold. It outputs the maximum packet rate the network can handle at various flow counts before violating the SLO latency. These thresholds are then fed into the long term optimization algorithm.




==> design_core.tex <==

% Flow-level load balancing is not practical for realistic traffic
% why not practical? what's the solution?

\section{\sysname's Design}
\label{sec:design}

In this section, we elaborate \sysname's design for supporting microsecond-scale tail latency SLOs efficiently.
We first summarize \sysname's key ideas. Then, we describe a high-level overview of \sysname, introduce critical system components, and explain them in details.

% Here are \sysname's key ideas.
Given our analysis on real-world traffic and NFV systems (\secref{sec:motivation}), we believe that \sysname's auto-scaling scheme must be able to \textit{detect and react to traffic bursts in a timely way for latency SLOs}, and \textit{consider fine-grained traffic statistics when assigning traffic to cores} for high CPU core efficiency. Specifically, \sysname's monitoring must provide traffic statistics at per-flow basis at short timescales (i.e. shorter than the timescale of a transient traffic burst), while being able to scale to hundreds of thousands of flows. \sysname's data-plane execution must work towards the Pareto frontier in the traffic space when many flows are processed at each core, and opportunistically utilize the multi-core pipeline mechanism to accommodate whale flows. \sysname's control-plane must make scheduling decisions in response to transient bursts in traffic rather than treating bursts indifferently via over-provisioning CPU cores. 

\subsection{System overview}
\label{subsec:system-overview}

% 0) system overview and components:
% - NFVCtrl, NFVCore & NFVRCore, NFVMonitor (for generating NF profiles)
% Need to mention: why these components are new and critical for our design

Next, we discuss \sysname's proposals in NFV's control-plane, the data-plane execution, and NF performance monitoring.

% \sysname is an NFV scheduler that runs NFV workloads on top of a rack-scale cluster. It runs NF chains, each with a target tail latency SLO. During the deployment of a chain, \sysname adapts to dynamic traffic to meet its associated latency SLO while ensuring high CPU core efficiency.

% To schedule an NF chain with \sysname, users need to provide an \textit{NF chain specification} which includes a description of NFs that \sysname should run and the way of forming a packet processing pipeline with these NFs.

\parab{\sysname's control plane.}
\sysname's control plane includes a \textit{hierarchical and hybrid} ingress and per-worker controllers.

\sysname's ingress distributes traffic for both inter-server and infra-server cases. It works at three different layers: at the ToR switch, at each server's NIC, at each CPU core associated with its own dedicated NIC RX/TX queue. \sysname's ingress works in hybrid mode, i.e. with both hardware and software forwarding, to achieve scalability and agility in the system's control-plane.

To scale to a large number of flows in real traffic, \sysname's ingress utilizes flow tables in hardware switches and NIC's RSS to route flow aggregates to distribute traffic loads in a (relatively) coarse-grained way. Further, it employs software-based forwarding to distribute bursts in traffic to nearby CPU cores when \sysname detects traffic bursts at a NIC's RX queue (associated with a core), and needs to migrate flows to avoid latency SLO violations.

At each multi-core worker, \sysname's controller manages the execution of NF chains and coordinates with the ingress.
It does so by interacting with other system components, including the NIC hardware and CPU cores.
Upon initialization, the controller configures the NIC hardware to create a pool of software queues, instantiates a pool of threads, each thread for running one or more NF chains.
Initially, NF threads are idle and not scheduled to run on cores.
At runtime, the controller is responsible to dispatch incoming packets into a number of NIC queues\footnote{The number of in-use NIC queues may be smaller than the total number of NIC queues at the system initialization.}, ensure each queue to be handled by one NF chain, and notify per-core thread schedulers to start running or stop running NF threads to scale up or scale down.

\parab{\sysname's data plane.}
\sysname's data plane provides mechanisms for handling bursts in traffic. It includes dividing CPU cores into two groups\footnote{We exclude the core for running the control-plane and management tasks.}, i.e. normal cores and sidecar cores, and splitting NF chains to enable a chain's pipeline mode in order to process whale flows when necessary.

\textbf{Normal core.} In \sysname, a normal core is associated with one NIC queue and one software queue. A normal core is responsible for 1) (periodically) pulling packet arrivals from the NIC queue designated to it and moving these packets to a number of software queues (w/ its own software queue preferred in this process); 2) running an NF thread, which does all required packet processing.

\textbf{Sidecar core.} Each server also reserves a number of sidecar cores. These sidecar cores do not own any NIC or software queues. However, they are responsible for processing software queues upon requests by \sysname's controller.
Software queues are owned by \sysname's controller, and are only borrowed by normal cores to absorb transient packet bursts. When a software queue is borrowed, a normal core starts to hand-off flows associated with the traffic burst. In the meanwhile, \sysname's controller seeks for an idle sidecar core, allocates the software queue to it, and then wakes up an NF thread on the sidecar core to process packets in the queue. Moreover, whale flows may exceed the processing capability of a single core. To properly process bursts caused by these flows, \sysname's controller may decide to let multiple sidecar cores to run one NF chain in the pipeline mode to increase the processing speed. However, splitting a chain across cores breaks the run-to-completion execution and leads to imbalanced loads, which produces a lower per-core throughput. Therefore, \sysname's controller must make decisions judiciously to avoid inefficiency in the execution of NF chains.

Each normal core has its designated NIC RX queue for receiving packets, and one local software queue, and a list of on-demand software queues. Both normal cores and reserved cores transmit packets through their own NIC TX queues after finishing the NF processing.

\parab{\sysname's performance monitoring.}
The performance monitoring component is to 1) provide necessary traffic statistics to help \sysname's control plane to make timely and efficient scaling decisions; 2) help generate an NF chain's short-term and long-term performance profile.

At runtime, \sysname appends a monitoring module to each thread running a chain. It maintains per-flow, per-core and per-flow-aggregate \textit{packet counters} and \textit{flow counters} at short and long timescales to support short-term and long-term scaling decisions.

When in profiling mode, \sysname's controller turns on the NIC's hardware timestamp. The monitoring module parses each packet's hardware timestamp prior to the NIC's TX function call, and computes per-packet worker delay, i.e. the total time that a packet has spent on the server (starting from the time arriving at the NIC's RX queue to the time departing from the NIC's TX queue). Details on generating an NF chain's performance profile are discussed in \secref{subsec:design-profiling}.


\subsection{\sysname's ingress: traffic assignment}
% why are we doing this:
% two different granularity of traffic assignment?

\sysname's ingress is to make traffic assignment decisions for incoming traffic.
In \sysname, a basic scheduling unit is a rack-scale cluster of servers connected to a ToR switch.
The ToR switch is the traffic ingress and egress. Traffic enters \sysname on a subset of ports; servers are connected to the remaining set of ports.


% high-flow rate makes it impossible to do per-flow routing at ToR
% software approach also suffers from the high latency
% In general, most stateful NFs maintain per-flow states, which requires \sysname's ingress to ensure flow-affinity.
% Thus, for stateful NF chains, the smallest load balancing unit is a single flow. 
% Prior work has proposed solutions that schedule individual flows \cite{wang2021galleon}. However, given a large flow rate (i.e. more than $10k$ flow arrivals per second), it is impossible to install a flow entry (at the ToR) for every new flow arrival.

% coarse-grained routing is bad for latency
% On the other side, a different thread of prior work ~\cite{sosp15-e2,nsdi18-metron,conext19-rsspp} proposes to utilize hardware to group flows (either via hardware hash function or via hardware flow table) at the switch and NIC hardware to split traffic into traffic classes or RSS buckets.
% The traffic assignment granularity is larger than the per-flow basis.
% However, this approach is affected by both types of traffic burstiness in \secref{sec:motivation}.
% We've shown that NFV systems are not able to meet tail (\pnintynine) latency SLO if they are affected by transient bursts in incoming traffic.

% we propose a combined hierarchical routing:
% coarse-grained at ToR and NIC; fine-grained at normal cores;
\sysname must employ a fine-grained per-flow assignment working at a microsecond-scale time granularity in order to detect and process transient traffic bursts timely.
Given our observations on the high flow rate and frequent transient bursts in real-world traffic, we propose a hierarchical ingress with a hybrid traffic assignment mechanism:
at the hardware (ToR and NICs), \sysname utilizes the hardware-aided hash-based flow grouping to split incoming traffic into many groups of flows, while each group finally arrives at a server's NIC queue, and is dequeued and processed by one normal CPU core.
For each normal CPU core, it also employs a software-based flow-level traffic assignment mechanism that detects transient bursts, and pin-points culprit flows. Once a burst happens, this software-based fine-grained assignment approach can borrow software queues from NFVCtrl, which then triggers the execution of NF threads on the set of reserved cores at a server. In this way, incoming traffic is split across the cluster, while transient bursts can be handled, without violating the flow-affinity constraint.


% 1) the fine-grained admission control to absorb transient bursts with reserved cores
\input{op_short}

% 2) the coarse-grained admission control to pack RSS-buckets into normal cores
\input{op_long}

% 3) the actual profiling approach
\subsection{Profiling: the approach and details}
\label{subsec:design-profiling}

\sysname's short-term and long-term optimizations use NF chains' performance profiles.
For each chain, \sysname generates a long-term and a short-term profile with an offline profiler.
According to measurements, a chain's latency distribution depends on two traffic factors, the number of active flows and the packet rate.
% There are other parameters like CPU frequency and cache size that can impact the latency but these parameters are fixed and hence not considered.
\sysname must consider both factors in the profiling process.

\parab{Long-term profile.}
To generate a chain's long-term profile, \sysname's profiler uses a traffic generator to control the traffic input with different number of active flows and packet rates.
It runs the chain with one core, and measures the end-to-end latency by serving traffic for 30 seconds.
To characterize the effect of \texttt{<flow count, packet rate>} on the chain's latency, \sysname searches the entire flow space.
Then, for a given target latency, the profiler produces a Pareto frontier in the flow space.
For a traffic input within the frontier, the core's \pninty latency is below the target.
% It outputs the maximum packet rate the network can handle at various flow counts before violating the SLO latency.

\parab{Short-term profile.}
Besides the traffic input, the short-term profile is related to the number of cores for running the chain. In \sysname, we consider NF chain splitting at the individual-NF level, and do not split a single NF into two sub-NFs.

The short-term profile requires \sysname to run with the long-term optimization but without the short-term optimization (i.e. by using zero sidecar core).
At each normal core, \sysname's monitoring component records \texttt{<flow count, packet count>}, i.e. the number of (processed) flows and the instantaneous (processed) packet rate, for each short-term epoch.
With many epoch records from normal cores, \sysname's profiler can generate the chain's short-term profile: given a flow count, it gives the average number of packets that a core can process within a short-term epoch.

Similarly, \sysname can produce the chain's profile for different chain-splitting schemes. It just has to replace each normal core with a normal core group (several cores running a chain in the pipeline) and repeat the above process.



==> design_general.tex <==

\section{NFV Deployment Challenges}
\label{sec:design-deployment-setting}

In this section, we describe \sysname's target deployment scenario, and clarify assumptions made in \sysname's design. We then discuss in details about problems in today's auto-scaling and load-balancing approaches. To achieve low-latency and high-efficiency in NFV, \sysname must propose solutions to address these, which we detail in \secref{sec:design}.

\subsection{\sysname's target deployment}
\label{subsec:deployment-setting}

To fulfill NFV's original ambitions~\cite{sigcomm14-making}, \sysname targets cloud-based NFV deployments, especially in the edge rack-scale cluster setting.
This setting is becoming more and more accessible and important because of the deployment of distributed edge cluster offerings and new latency-critical applications at the Internet edge (\secref{sec:intro}).

In this context, \sysname is designed to host and schedule NFV workloads on top of a cluster with one or more racks of machines.
NFs perform packet processing tasks in sequence on traffic. This sequence of NFs is called an NF chain.
To meet different network service needs, many NF chains can co-exist in a single cluster.
To deploy a specific NF chain, \sysname's users must submit a set of NFs and the order in which they are applied to traffic (usually a traffic class). Then, users may submit multiple NF chains to be deployed by \sysname to serve different classes of traffic.

NF chains perform different computations on packets, and have different performance requirements (e.g., latency SLOs).
\sysname must allocate enough computing resources to each chain to meet their requirements.
Due to dynamic traffic, each NF chain can also have different requirements on its allocated computing resources over time, thus it can be associated with one or more servers in the cluster.
Note that we make the assumption that each server runs only a single NF chain.
This is reasonable because:
a) given a high traffic volume, an NF chain is likely to expend to cores on multiple servers;
% b) multiple NF chains may contend with each other on shared resources, when they share the same server. ResQ~\cite{nsdi18-resq} has studied the case and proposed a solution to optimize each server's aggregated throughput, which can be applied in \sysname if necessary;
b) spare resources can be allocated to background tasks (e.g., garbage collection tasks) or other latency-insensitive tasks (e.g., batch processing). Prior work~\cite{nsdi19-shenango} has explored this design to improve the overall system's efficiency.


Note that in \sysname, a subset of CPU cores is reserved as \textit{sidecar} cores.
These cores are used for processing traffic bursts for NF chains.
They are mainly used for other latency-insensitive applications if it is not notified by \sysname's per-worker scheduler to process traffic bursts. We will discuss this design in detail later.


In \sysname, each server has at least one \textit{data-plane NIC} to receive traffic for NFV processing. \sysname's auto-scaling works for infra- and inter-server scaling to ensure that traffic is spread out across cores in each server and across servers.


\subsection{Problems on existing approaches}
\label{subsec:problem-on-us-slo}

NFV systems have auto-scaling or load-balancing schemes to adjust resource allocations in response to load changes in traffic. Some systems do not explicitly consider latency objectives, and then fall short in meeting microsecond-scale latency SLOs~\cite{conext19-rsspp}. We omit these in our following discussions. For other NFV systems that do consider latency, they are limited by the following issues.

% <Briefly show experimental results that validate this>.
\begin{figure}[t]
\begin{center}
\resizebox{0.8\columnwidth}{!}{
    \includegraphics[frame]{figs/latency_cdf_flow_count.png}
}
\caption{Latency distributions of serving traffic with one core under different number of active flows in the traffic. As the number of flows increases, the latency distribution moves towards right (i.e. higher latency).}
\vspace{-2mm}
\label{fig:nf-profile-flow-count}
\end{center}
\end{figure}

\parab{Inappropriate choice of scaling signals}.
They use traffic rate estimates (e.g., packet and bit rates) as signals for auto-scaling and load-balancing~\cite{conext20-lemur,nsdi18-resq,socc20-snf,wang2021galleon}.
Using traffic rate estimates can cause problems when targeting microsecond-scale SLOs for three reasons.

First, traffic rate estimates are often calculated as the moving average values, updated periodically every 100s milliseconds or even a few seconds. This means that rate estimates are updated not only in a less timely manner, but also in a way that omits necessary details about transient bursts in traffic.

Next, some systems~\cite{sosp15-e2,nsdi18-metron,wang2021galleon,socc20-snf} utilize a cluster-level controller to make scaling decisions based on remote traffic statistics (such as packet rates and latency estimates). These remote scaling signals may be suitable to support coarse-grained scaling decisions, however, they can introduce new sources of delay in the measurement-reaction loop, which prevents the controller from reacting timely to transient bursts observed by CPU cores across the cluster.

Lastly, our measurement (\secref{sec:motivation}) shows that it is important to consider the number of flows when serving traffic at a core. Put it differently, the processing capacity of a core is limited both by the current traffic rate and the number of flows that have arrived within a time window. The intuition is that as most stateful NFs have per-flow states, having more flows can reduce the cache efficiency at a core, which in turn increases the latency even if the traffic rate remains the same. \figref{fig:nf-profile-flow-count} demonstrates this by showing CDF curves under different numbers of active flows when serving the same traffic volume with one core.



With above observations, we notice that there is a Pareto frontier in the space of \texttt{\small <flow count, traffic rate>}, for serving traffic with a given CPU core and under a target \pfifty or \pnintynine per-core latency.
Then, Ironside must take both factors into consideration when its auto-scaling algorithm adjusts core allocations to either pack loads to fewer cores or scale out persistent load changes and transient bursts to more cores.
Further, to adapt to transient bursts in traffic, the scaling signal must be able to capture these bursts, which cannot be a remote signal or a moving-average value.
All these considerations have been ignored by prior work.


\parab{Insufficient scaling time granularity}.
In \secref{sec:motivation}, we have shown that transient bursts can happen at both short timescales (less than 10 ms) as well as at longer timescales, while transient bursts at short timescales cause the most SLO violations. They affect a significant fraction of incoming traffic, which places a fundamental difficulty in meeting microsecond-scale tail latency for NF chains.
We believe that it is impossible to achieve microsecond-scale latency SLOs without properly handling transient bursts, especially bursts in short timescales.

Previous systems all run auto-scaling or load-balancing in time granularity of 100s-1000s milliseconds, which can be two orders of magnitude larger than the time scale of transient bursts.
As a result, these systems fail to detect transient bursts and react to them. So, they do not handle them properly to prevent SLO violations. 
Therefore, \sysname must employ mechanisms to efficiently detect and absorb transient bursts in traffic at active CPU cores.

\subsection{Insights on achieving high CPU efficiency}
\label{subsec:strawman-solution}
The above discussion is on achieving microsecond-scale tail latency SLOs. However, one can design a system that over-provisions computing resources, which can waste a significant amount of resources and be impractical for real deployments.

As discussed in \secref{sec:intro}, \sysname aims for both low latency and high efficiency.
Before diving into the detailed design of \sysname, we look at several strawman solutions for meeting microsecond-scale tail latency SLOs.

\parab{Static allocation}.
An NFV system may allocate cores conservatively \textit{statically for all time}. In this context, the control-plane can spread out flows conservatively to all CPU cores in the cluster; cores may run in the pipeline mode to accommodate whale flows (this is necessary according to our analysis \secref{sec:motivation}), so that every core is well prepared for the worse case delay give the flow assignment.

\parab{Scaling only in the long term}.
Alternatively, an NFV system can turn on auto-scaling in long timescales, but do not have explicit mechanisms to detect and process transient bursts that happen in short timescales. Then, cores need to be allocated conservatively to avoid SLO violations in short timescales, while the control-plane adapts cores gradually in response to persistent load changes.

\parab{Scaling without optimal packing}.
At this time, the system chooses to adapt over both timescales, and has a mechanism to detect and process traffic bursts. It uses both short-term and long-term optimizations to try to minimize the CPU core usage by dynamically re-grouping flows to cores. However, without considering flow counts and individual flow sizes, this approach may lead to over-provisioning because its scaling algorithm must pack flows conservatively.

% We evaluate these in \secref{sec:evaluation}.

 


==> design_outline.tex <==
Setting/assumptions:
- a cluster with several racks
- a set of NF chains deployed on the cluster
- each NF chain is associated with one or more servers in the cluster
- a server runs only a single NF chain (spare resources can be allocated to background/other tasks).
- incoming traffic is split across cores in the server
- slight issue: we need to set aside reserved cores; discuss this later.

Previous systems use packet rate estimates for auto-scaling and load-balancing.

Section 2 shows that the number of flows is also important. In other words, the capacity of a core is limited both by the packet rate and the number of flows. Intuition for this: NFs have per flow state, and having more flows can reduce cache efficiency, which can in turn increase latency. <Briefly show experimental results that validate this>.

So, for a given CPU core and for a target p50 or p99 core, there is a Pareto frontier in the space of <#flows, packetrate>. Ironside makes CPU allocation decisions for flows (i.e., mapping flows to CPUs) based on both of these factors; no prior work has observed this.

Section 2 also shows that transients in <#flows, packet-rate> can also happen at very short timescales (10s to 100s of us) as well as at longer timescales.

Strawman:
- allocate cores conservatively statically for all time (may need a large number of cores)
- allocate cores conservatively for short-time scales, but adapt over longer timescales
- adapt over both timescales (the last can minimize CPU usage).

Ironside approach:
- in the short timescale, use /sidecar/ cores to process bursts
- in the longer timescale, re-allocate flows to cores
Both of these make allocation decisions based both on the number of flows and the packet rate.



==> intro.tex <==

\section{Introduction}
\label{sec:intro}

% Jianfeng: do we need this paragraph?
% - Tail latency for RPC protocols is handled in software, right?
% sosp17-zygos,shinjuku-nsdi19,nsdi19-shenango,osdi20-caladan
% router: old packet-switching papers
% end-host: Swift
% RPC protocols: not true
% Datacenter RPCs can be General and Fast [NSDI '19]
% networking.

% What are NFs and what are NFV?
% NFV deployment scenario
Network Functions (NFs) process packets in NF chains, and are increasingly key for networking in edge clouds.
Network Function Virtualization (NFV) and software-based packet processing has expedited the development of new NFs and eased the management burden previously borne by a generation of network operators~\cite{sigcomm14-making,sosp15-e2,osdi16-netbricks,sigcomm17-nfp,sigcomm17-nfvnice,nsdi18-resq,socc22-quadrant}.
However, the performance of software-based NFs remains a core drawback of NFV. The community has once again sought to move processing to hardware, this time programmable or flexible in the NFs that can be run. Given the limited generality, flexibility, and large-scale deployability of specialized programmable hardware devices, hardware offloading still leaves critical and complex NF processing in software, or requires a very specific solution for certain classes of NFs~\cite{eurosys15-nba,socc17-uno,conext20-lemur,osdi20-pigasus}.
% Moreover, NF deployments can often involve many cloud providers with different assumptions on their underlying infrastructure, which makes bespoke hardware offloading solutions even hard to be adopted. 
In this paper, we focus on NFV deployment scenarios at the edge \textit{rack-scale} cluster, where one or many software-based NF chains are hosted to process different traffic classes.

For decades, the community has studied how network nodes can perform processing within a short time budget~\cite{1995-guaranteed-service-network,1996-bounded-delay,sigcomm20-swift}.
% This question has dominated router design~\cite{1995-guaranteed-service-network,1996-bounded-delay}, end-host stacks~\cite{sigcomm20-swift}, RPC protocols~\cite{}, and far more~\cite{}.
It was long the case that only specialized, limited-functionality hardware was up to the task.
Prior work has shown that commodity processors can process moderately-complex NF chains at line rates and adjust core allocations dynamically to match traffic demands~\cite{nsdi18-metron,conext19-rsspp,conext20-lemur,socc20-snf,socc22-quadrant}. Among them, some employ \textit{auto-scaling} to ensure CPU core efficiency while minimizing packet losses and optionally meeting latency SLOs. Others have explored \textit{load-balancing} mechanisms that assign traffic to cores to minimize load imbalance but do not consider latency explicitly.


% we need low-latency, because of new critical applications

NFV must provide small tail latency SLOs because \textit{the execution of NF chains is pure overhead}. Low-latency SLOs enable service providers to offer tighter end-to-end SLOs for applications, especially
with the development of edge rack-scale cluster offerings~\cite{gcp-distributed-cloud} and latency-critical applications, such as autonomous driving, AR/VR, and 360\textdegree ~video~\cite{hotnets2020:pruning-edge-research}.
As processor speeds increase, most NFs can complete their processing within tens of microseconds. Ideally, latency SLOs should be a small multiple (10-100x) of the total processing time for an NF chain, allowing queueing at a moderate level. Given the need for real time responsiveness in these emerging applications,  NFV must meet microsecond-scale tail (\pninetynine) latency SLOs.

\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
% \vspace{-6mm}
\begin{table}[tb!]
\resizebox{1.0\columnwidth}{!}{
\footnotesize
\centering
\begin{tabular}{|m{1.8cm}||M{1.6cm}|M{1.4cm}|M{1.1cm}|M{1.7cm}|}
% \begin{tabular}{|m{1.6cm}||c|c|c|c|}
\hline
\textbf{Framework} & Control-plane Scalability & Burst-aware Scaling & Agility &  Burst-handling Mechanism \\
\hline\hline
\sysname & \cmark & \cmark & \cmark & \cmark \\
\hline
Metron~\cite{nsdi18-metron} & \cmark & \xmark & \xmark & \xmark \\
\hline
Quadrant~\cite{socc22-quadrant} & \xmark & \xmark & \xmark & \xmark \\
\hline
Dyssect~\cite{infocom22-dyssect} & \cmark & \xmark & \cmark & \xmark \\
\hline
\end{tabular}
}
\caption{A comparison of NFV platforms' auto-scaling and load-balancing properties that are key for achieving microsecond-scale tail latency.}
% \vspace{-1em}
\label{t:nfv-scaling-comparison}
\end{table}

Unfortunately, today's auto-scaling and load-balancing approaches exhibit poor latency-sensitive performance. For real traffic, they require orders-of-magnitude larger tail latency SLOs. Our analysis of traffic behavior indicates that there exist two key traffic patterns that are ignored by prior work: (1) \textbf{whales}: large flows whose processing capacity exceeds a core; (2) \textbf{schools of minnows}: a large number of small flows \textit{concurrently} arriving at a core. These traffic patterns can cause long-lived or transient long packet queues that lead to tail (\pninetynine) latency of several (tens of) milliseconds (\secref{sec:motivation}).


There are three drawbacks to existing NFV auto-scaling and load-balancing approaches.
First, \textit{insufficient load distribution}: NFV systems typically use poll-mode user-space networking (e.g., with DPDK~\cite{dpdk}) and run-to-completion for high per-core performance~\cite{nsdi18-metron, nsdi18-resq, socc22-quadrant, atc20-edgeos}. Prior to actual processing, traffic is split into queues in two ways:
(1) using an ingress that routes each flow to a core, collecting coarse-grained statistics (e.g., a moving average of per-flow rates), which is insufficient to capture transient bursts in traffic;
% A pure software-based ingress can also has limited scalability and high overheads of packet forwarding.
(2) routing flow aggregates (e.g., RSS-based systems), which scheme scales but does not take flow counts or individual flow sizes into account, and fails to adapt to load changes at small \textit{traffic scales}. Second, \textit{coarse-grained decisions}:
existing NFV systems make scaling decisions at a coarse time granularity, from hundreds of milliseconds to seconds, due to the use of hardware forwarding or remote ingress.
% Some  use flow tables at hardware switches~\cite{wang2021galleon}, which then exacerbates the latency problem because of the slow flow installation delay (100s milliseconds) at hardware switches.
However, we show that most SLO violations are transient violations that occur at small timescales ($<$10 milliseconds) (details in \secref{sec:motivation}).
Third, \textit{no burst-handling mechanisms}: existing systems optimize for the average case for the median latency\barath{What does "average case for the median latency" mean precisely? Can we rephrase to make it simpler/easier to understand?}, but lack special mechanisms that deal with the worst case in a different way.
As a result, under the peak load, traffic arrives at a queue as a large burst that can still lead to tail-latency SLO violations, even if there are nearby underutilized cores; under normal loads, a core polls its designated queue but only sees very few packets.
Therefore, cores can waste CPU cycles without performing any useful processing, but still suffer tail-latency SLO violations.
% This phenomenon becomes more significant under microsecond latency SLOs.
In fact, we show that for some NF chains, it is impossible to meet microsecond tail-latency SLOs without optimizing for the worst case.
In \tabref{t:nfv-scaling-comparison}, we compare \sysname against other existing NFV systems with alternative auto-scaling or load-balancing schemes.


In this paper, we describe the design and implementation of \sysname, a rack-scale NFV cluster scheduler meets microsecond-scale tail latency SLOs with high CPU efficiency by addressing the problems we listed above.
In \sysname, the key challenge is to \textit{dynamically assign flow aggregates to cores while tracking flow sizes and counts at fine traffic and time scales to achieve timely burst mitigation with low overhead}.

\parab{Contributions}. We make the following contributions.

% NFV workload specific observation

% While datacenter applications have required microsecond-scale guarantees~\cite{sosp17-zygos,nsdi19-shenango,osdi20-caladan,osdi20-breakwater}, NFV systems have yet to achieve high packet rates under microsecond-scale tail latency (e.g., the \pnintynine percentile) requirements.

% To service providers, NFs represent a unique workload that is fundamentally different from normal cloud applications: each incoming packet triggers a series of NF computations, forming an \textit{NF chain}; each NF chain processes a traffic class consisting of many flows or sessions under a strict end-to-end \textit{per-packet} Service Level Objectives (SLOs); NFs process raw packets instead of application requests that may span across several packets; the packet processing time and the packet transmission time are on the same level as a microsecond-scale latency SLO, which greatly limits the amount of queueing allowed at each individual queue in the system. These differences limit the possibility of reusing design principles tailored for microsecond-scale RPC systems, and call for a new cluster design that targets for executing packet processing tasks under low-latency requirements.

% Further, existing NFV systems have focused on customizations for achieving high performance (i.e. low latency and high throughput), but ignore the importance of doing so efficiently. We argue that efficiency is an important aspect of an NFV system, because NFV represents a large-footprint workload at the Internet edge with limited computing resources~\cite{conext20-lemur}.

% We ask: is it possible for an NFV system to get the best of both worlds: high performance and high efficiency, when hosting microsecond-scale NF chains? Existing NFV systems fall short in meeting this goal for several reasons.
% The system scales up and down each NF chain to serve dynamic traffic under a microsecond-scale latency SLO, and aims for the best of both worlds: high performance and high efficiency

% What is the problem with the current NFV solution
% 1) the packet processing time is at the same level of the network transmission time
% 2) the latency SLO is only several times of the packet processing time
% 3) queueing causes the super-high tail latency that is 1000 times larger than the median end-to-end per-packet latency


% Second, today's NFV systems do not consider hardware queues in the network. Even though high-speed networks today provide round-trip (RTTs) on the order of a few $\mu$s, packet queues built up by packet arrival bursts can lead to 10-1000$\times$ delays in the worst cases. As the per-packet processing time gets close to the network transmission time of a packet, it is important to take the in-network hardware\barath{Is it just hardware queueing that we care about?} queueing into account when balancing loads across servers in a cluster.

% This leads to an inefficient execution of NF chains: as an NFV system must meet tail latency SLOs for these chains, it must limit the amount of traffic aggregates (e.g., flows) processed by an NF chain running on a core. This forces it to split traffic across many busy-polling CPU cores, while these cores are not being fully utilized for most of the execution time.

% The state-of-the-art NFV systems utilize fast user-space networking, such as DPDK\cite{dpdk}, for efficient packet I/O. They run each NF in the polling mode that dedicates a CPU core and a packet queue to it. Recent efforts propose to execute an NF chain in the run-to-completion way and use multi-queue NICs (e.g. using flow tagging at the ToR switch). They all try to keep a consistent mapping of flows to queues (and then to cores).



% \parab{Identify the tail latency challenge}.
% For real traffic, we identified challenges of meeting tail latency SLOs when serving NF chains: an NFV system's tail latency is affected by both long-term overloads and short-term traffic bursts. Our measurement study demonstrated that an NFV system cannot meet the tail latency SLO unless it employs special mechanisms to handle transient traffic bursts properly.

\parae{Hierarchical Hybrid Ingress}.
\sysname's use of hierarchical and hybrid ingress ensures both scalability and the ability to react to traffic bursts at fine traffic and time scales. The ingress follows a hierarchical design: at the inter-machine layer, it collects coarse-grained traffic and performance statistics and forwards traffic based on flow aggregates for high scalability and efficiency; at the intra-machine layer, the ingress works in hybrid mode: by default, it uses NIC flow tables and RSS to split traffic. It also adds fine-grained per-flow packet-level traffic statistics, and promptly redirects traffic in software whenever a burst is detected at a core.

% traffic-aware packet/core (network/cpu) scheduling mechanism. It detects transient traffic bursts in the incoming traffic, and works within a microsecond-level time granularity. At the end of each epoch, the algorithm determines the additional number of CPU cores for absorbing transient bursts at each NIC queue, and multiplexes additional NFV threads among a pool of reserved CPU cores.

\parae{Burst-aware Scaling}.
\sysname's burst-aware scaling algorithm is key for auto-scaling with micrsecond-scale tail latency SLOs. Unlike previous systems, \sysname's scaling algorithm includes both long-term and short-term optimizations. Its long-term optimization runs every 100s milliseconds\barath{Is this supposed to say "100" not "100s"?} to re-balance loads across cores to adapt to persistent load changes to ensure CPU core efficiency. Its short-term optimization works at a fine timescale (smaller than the target latency SLO) to only scale out in response to traffic bursts that are detected between two long-term optimizations. Note that the short-term optimization uses packet counters rather than long-term traffic rate statistics (such as packet rates). \sysname uses NF performance profiles that consider both packet and flow arrivals/departures to tightly pack loads.

% To do so, the scaling algorithm uses hardware timestamping to model per-packet latency given a traffic input. It uses this model to help formulate the scaling problem, and solves the optimization problem to set NIC’s RSS function to balance loads among the set of active normal CPU cores, while keeping the P99 latency  \textit{close} and \textit{below} the target latency SLO. This scaling algorithm keeps each active core as busy as possible without latency violations, which improves the system’s efficiency.

\parae{Dynamic NF Chain Splitting}. \sysname's chain-splitting mechanism handles transient bursts explicitly: besides CPU cores for processing normal loads, \sysname sets aside a subset of CPU cores on each machine as \textit{sidecar} cores to just process bursts. Sidecar cores are not assigned with dedicated NIC queues. They are only responsible for processing packets in software queues sent by other normal CPU cores. When a burst arrives at a normal core: if many small flows cause the burst, \sysname \textit{splits flows into software queues}; each can be handled by a sidecar core without SLO violations. If large flows cause the burst, \sysname \textit{splits chains into multiple cores} so that cores can work in pipeline mode to handle large flows without SLO violations.

We have implemented \sysname, and evaluated it by hosting canonical NF chains to serve traffic in a rack-scale cluster. We find that our system outperforms state-of-the-art NFV systems in both latency and efficiency~\cite{infocom22-dyssect,nsdi18-metron,socc22-quadrant}: 1) \sysname is able to meet microsecond-level tail (\pninetynine) latency SLOs, which existing NFV system with alternative auto-scaling approaches cannot achieve; 2) by setting our tail latency SLO to other NFV systems’ P50 latency, our system uses X\% less time-averaged CPU core. This means that \sysname’s auto-scaling is able to improve CPU core efficiency for NFV.



% \barath{We need to end the intro on a slightly stronger note, but I'm not quite sure yet.}






==> intro_outline.tex <==
An Outline of the paper's introduction

Title: Ironside: Microsecond-scale Latency SLOs for Network Function Chains

NF-chain processing has received much attention in the literature
- explain NFs and NF-chains briefly

Prior work has shown that commodity processors can process moderately complex NF chains at line rates by auto-scaling core allocations to match traffic demands.
- Auto-scaling approaches attempt to ensure CPU efficiency while (optionally) meeting tail latency SLOs.
- (Aside: other work has explored /load-balancing/ techniques that assign cores to traffic while minimizing the number of cores. They do not explicitly consider latency).

Latency SLOs for NF chains needs to be small. NF chain execution is pure overhead, and smaller SLOs will enable the provider/telco to offer tighter end-to-end SLOs for applications:
- especially important for latency-sensitive applications in edge rack cluster deployments

How small should latency SLOs be?
- as processor speeds increase, many NFs can complete within a few (tens of) microseconds
- ideally latency SLOs should be a small factor (5-10x) of the total processing time for an NF chain
- hence /microsecond-scale latency SLOs/

However, existing auto-scaling/load-balancing approaches do not perform well (can require large latency SLOs) for two types of traffic patterns present in real traces:
- large flows whose processing capacity exceeds a core (whales)
- a large number of small flows concurrently arriving at a core (school of minnows)
Such traffic patterns result in transient or long-lived large queues that can result in p99 tail latency of several milliseconds (or nearly 100x NF chain processing time)

Why don't existing auto-scaling/load-balancing approaches do well?
- One class of approaches: RSS-based systems or those that route flow aggregates do not take number of flows or individual flow sizes into account
- Quadrant/SNF: route each flow to core; as the number of flows increases, then the ingress is unable to keep up with routing
- Most systems make decisions at 100~ms granularity; many transient SLO violations occur at very small timescales (6~ms).

Key challenge:
- (dynamically) *assigns flow aggregates to cores*, but also *tracks flow size and number of flows* at *fine timescales* and *without incurring high overhead*

Contributions:
- <how does Ironside solve each one of these problems>


==> motivation.tex <==

\section{Motivation}
\label{sec:motivation}

% what do we want to discuss in the motivation section?

% Our main focus is to find the set of mechanisms that is key for achieving high efficiency while meeting tail latency SLOs.
In this paper, we focus on \textit{auto-scaling}.
An NFV system uses the auto-scaling mechanism to adapt to dynamic traffic.
Auto-scaling is responsible for:
1) determining the set of active CPU cores in the cluster and distributing traffic among them;
2) detecting overloaded CPU cores and migrating excessive traffic from these cores to prevent latency SLO violations.

% Before we discuss the detailed system design, we introduce several key observations drawn from NFV systems when hosting stateful \nfchains to several realistic traffic.
% These observations are crucial to understand the often-ignored challenges in achieving both low latency and high efficiency for NFV systems.

The system community has studied auto-scaling mechanisms for scheduling RPC workloads to achieve low latency and high CPU efficiency~\cite{sosp17-zygos,nsdi19-shenango,osdi20-caladan,osdi20-racksched}.
These solutions (e.g. JSQ scheduling) can be applied to \sysname for stateless NF chains.
Hence, deploying stateless NF chains is trivial in \sysname.
However, as most useful and critical NFs are stateful NFs, \sysname must focus on stateful NF chains. We find supporting microsecond-scale tail latency SLOs for stateful NF chains is non-trivial in an NFV system, because of the \textit{flow affinity} constraint.

\parab{The flow affinity constraint.}
Most stateful NFs have per-flow states~\cite{nsdi17-stateless}. A new NF state is created upon a new flow arrival and updated by the NF chain instance associated with the flow.
% Multi-flow and all-flow states do exist, and they can be partitioned into several NF instances running on their dedicated CPU cores, updated locally and and synchronized periodically under different consistency requirements with the assistant of the NFV system’s control-plane~\cite{sigcomm16-openbox,nsdi-18-s6}.
The flow affinity constraint is defined as: for a stateful NF chain, packets of the same flow need to be routed to and processed by the chain instance (running by a specific core) with the flow's corresponding NF states.
\sysname must consider this constraint rather than applying a general task scheduling scheme (e.g., JSQ scheduling), which may forward packets from the same flow to different cores and trigger frequent NF state synchronization across cores in the cluster.
In contrast, task scheduling for RPC workloads is not limited by the flow affinity constraint because RPC requests are not correlated.
Thus, \sysname cannot simply borrow ideas from previous efforts on task scheduling for RPC workloads.


% introduce the setting our measurement study
We conduct a simulation study to quantify the difficulty of achieving microsecond-scale tail latency SLOs and high efficiency while considering the flow affinity constraint.
We use a packet-level discrete simulation framework.
The framework simulates a rack-scale NFV system, including one ToR switch and many multi-core servers.
It takes a realistic traffic trace as input, replays the trace and direct traffic to the simulated cluster running NF chains.
Without losing generality, we use two different packet traces: one is a city backbone trace~\cite{}; the other trace is collected in a large autonomous (AS)~\cite{}.


% second, the measurement result of two types of burstiness
\subsection{Motivation against no burst-handling mechanisms}
\label{subsec:burst-in-real-traffic}
\jianfeng{I need to revise this part}

The flow affinity constraint requires an NFV system to distribute traffic at least at the per-flow granularity.
It leads to two types of traffic bursts at a core:
1) \textbf{whales}: a few large flows whose instantaneous packet rates may exceed a core's processing capacity;
2) \textbf{schools of minnows}: a large number of small
flows concurrently arriving at a core.
Next, we describe motivation cases on effects of the two types of traffic bursts.

% I repeated the one-flow-per-core experiment by using the three traces and increasing the per-packet processing time up to 20 us.

% I repeated the N-flow-per-core experiment by using the synthetic traffic, which has a various # of flows at a fixed packet rate. In the simulation framework, I implemented a flow generator that can generate traffic with different numbers of flows at a fixed aggregated packet rate (flows have the same average packet rate, and flow duration).

% Original data:
% a table that shows the tail latency results
% for different NF chains under different traffic inputs.

First, we set a large number of cores in the simulation framework so that each flow can be processed by a core.
We report the tail (\pnintynine) latency results produced by the simulation framework.
Even with unlimited CPU cores, the overall tail latency still goes up to 0.448-3.718 ms (x89.6-x185.9 of the per-packet processing time) for the backbone trace.
For serving the AS trace, the overall tail latency is also increased to 15 ms for a heavy NF chain (i.e. 20 us per-packet processing time).

Then, we run NF chains to serve synthetic traffic produced by a traffic generator, and find the P99 latency increases as the number of flows per core increases.
We also collected the median and the \pnintynine number of active flows at a core.
Our simulation suggests that each core may serve up to 5200 flows for the backbone trace.
For heavy chains (per-packet processing time >= 5 us), the P99 latency is expected to be >500 us when many flows.
% For light chains (per-packet processing time < 5 us), the P99 latency is expected to be at multi-10 us.


% Google Doc: Oct. 25th, 2021
% Targeting a 90% per-core rate leads to 750+ concurrent flows per core at median.
% At each core, the flow counts vary significantly. (P99 flow count > 2 x P50 flow count).
% One can control the per-core flow count at the tail. However, it can reduce the system’s efficiency

With practical considerations, most NFV systems with auto-scaling distribute traffic in flow aggregates to utilize hardware resources at the switch and NICs for forwarding packets.
For these systems, the auto-scaling mechanisms do not consider flow counts or individual flow sizes, and thus can neither detect nor react to the two types of traffic bursts.
This prevents them from meeting microsecond-scale tail latency SLOs.

% Some work at the per-flow granularity with a system-level ingress working with remote traffic statistics from servers.

% TODO(Add system benchmark results)
% Google Doc: Dec.13th 2021
% High rate flows cause a high tail latency for a heavy chain (i.e. chain #2, >12000 cycles per packet, or 7 us)
% For the other three chains, they are either a lightweight stateless or stateful chain that simply requires 1-3 hash table lookups for a packet (i.e. <1500 cycles per packet,  0.9 us). The high rate flow does not cause a high tail latency for them.
% Accelerating the trace makes chain #2 performance worse. However, it does not affect the latency results for the other three chains


% first, the measurement result of burstiness duration and affected packets
\subsection{Motivation against a coarse-grained scaling}
\label{subsec:sources-of-violations}

Next, we study a canonical NFV auto-scaling scheme.
In this scheme, the NFV system has a traffic ingress that distributes traffic to cores, while each core adopts the run-to-completion execution to run an NF chain instance.
The ingress routes traffic aggregates based on flow hashes to cores, and enforces flow affinity by maintaining a flow table.
In this experiment, we adjust the number of cores so that the simulated NFV system can control the median per-packet latency under the target latency SLO 200 $\mu$s. Lastly, we notice the tail (\pnintynine) per-packet latency is more than 6 ms, which is 30$\times$ higher than the target latency.

To further investigate the high tail latency, we collected system logs at the time granularity of 200 $\mu$s from each CPU core in the cluster.
For each 200-$\mu$s epoch, the log records per-packet delay for packets processed by each core in the epoch.
For each core, an epoch is called \textit{SLO-violating epoch} if there is at least one packet whose delay exceeds the target SLO.
In general, SLO-violating epochs are caused by a large packet queue, and tend to appear as a series of consecutive epochs.
For a series of consecutive SLO-violating epochs, we call it a SLO-violating event.

We study the time period (in epochs) of all SLO-violating events and find that:
among all latency SLO violation events, the \pnintynine percentile of the event length is 34 epoches (i.e. 6.8 ms). For simplicity, we define a transient SLO-violating event as an event whose time duration is less than 10 ms. A persistent SLO-violating event is a SLO-violating event whose time duration is more than 10 ms. We find that: transient \textit{(rather than persistent)} SLO-violating events have the dominant effect on the system's tail latency, and affect 3-4\% of total packets.
Unfortunately, existing auto-scaling approaches are too coarse-grained in timescales (hundreds of milliseconds to seconds) so that they are insufficient to detect and process transient SLO-violating events.

% # of short-term SLO-violation epoches
% # of packets affected by short-term SLO-violation epoches
% 99% SLO violation events happen within 6.8 millisecond (i.e. 34 epochs);

% Define:
% A persistent SLO violation keeps at least 10 millisecond;
% A temporal SLO violation keeps less than 10 millisecond;

% persistent violation event 1.15%
% transient violation event 2.18%

% A brief summary

\parae{Summary.}
Today's auto-scaling approaches are insufficient to achieve microsecond-scale tail latency SLOs.
On the one hand, these approaches are too coarse-grained in both the traffic and time granularity when distributing traffic to cores under the flow affinity constraint.
Our simulation results show that:
without handling properly, transient bursts in small timescales could cause tail latency SLO violations.
On the other hand, these approaches are not burst-aware, and lack mechanisms to adapt computing resources to deal with the two types of bursts in traffic.


% We believe that an NFV system must employ fine-grained scaling mechanisms that devote system resources quickly so that transient traffic bursts can be handled properly, in order to meet a tight tail latency SLO.

% then, what is the source of inefficiency in an NFV system?
% \subsection{Sources of system inefficiency}
% \label{subsec:sources-of-ineffi}
% Sources of NFV system’s inefficiency






==> op_long.tex <==

\subsection{Auto-scaling with the long-term optimization}
\label{subsec:long-term-op}

\sysname needs to adapt to load shifts that happen at each normal core with a dedicated NIC RX queue. As the other part of \sysname's auto-scaling, the goal of \sysname's long-term optimization is to \textit{minimize CPU core usage without overloading cores by persistent traffic load changes}. It does so by re-balancing traffic loads across normal CPU cores periodically. With a NF chain's long-term performance profile, it runs periodically to decide the number of normal cores and adjust the traffic assignment.

% \sysname's uses a hierarchical and hybrid ingress.
\sysname's long-term scaling algorithm works at the flow-aggregate level and runs at a much larger time granularity\footnote{We use the default time granularity of 100 milliseconds, which is determined by the flow installation time at hardware switches and NICs}.
At this stage, \sysname assumes that transient traffic bursts can be handled well by its short-term optimization (\secref{subsec:short-term-op}).
The long-term optimization utilizes flow tables and the RSS feature at the NIC and the ToR switch. It groups flows into RSS buckets, and assigns each individual RSS bucket to a CPU core.
Suppose that any SLO violations within a RSS bucket and in between two long-term scaling events can be handled by \sysname's short-term mechanism.
\sysname's long-term optimization only has to determine the set of normal cores that is enough for serving the current traffic without SLO violations caused by persistent traffic changes.

% discuss how we can maintain the RSS-bucket statistics by using the NIC feature

\parab{Inputs from measurements.} \sysname's long-term  optimization takes as input real-time measurements updated for every long-term epoch.
In a long-term epoch, \sysname maintains the cumulative number of packets and the active flow count seen per RSS bucket. As each normal core may see packets that belong to multiple RSS buckets, \sysname utilizes a NIC feature that tags each packet its own RSS hash value to the per-packet metadata field. Then, per-bucket packet counters are converted to per-bucket packet rates, which are related to latency targets according to NF chain's performance profiles.

\begin{table}[tb]
\centering
\normalsize
\resizebox{\columnwidth}{!}{
    \small
    \begin{tabular}{|p{3.0em}|p{5.2em}|p{14.8em}|}
    \hline
    Symbol & Type & Description \\
    \hline
    \hline
    $F$ & Integer & Total number of \textit{buckets} \\
    \hline
    $C$ & Integer & Total number of \textit{normal cores} \\
    \hline
    $BR$ & Real[$F$] & Packet rate per \textit{bucket} \\
    \hline
    $BF$ & Integer[$F$] & The number of active flows per \textit{bucket} \\
    \hline
    $X$ & Constant & The upper-bound of the number of active flows at a \textit{normal core} \\
    \hline
    $CPU$ & Binary[$C$] & Indicator array for CPU core states. \textit{Core} $i$ is active if $CPU[i]$ is true \\
    \hline
    $M$ & Binary[$C$][$F$] & Mapping between \textit{cores} and \textit{buckets}: bucket $j$ is assigned to \textit{core} $i$ if and only if $M[i][j]$ equals 1 \\
    \hline
    $T$ & Real[$X$] & Given a flow count $X$, the packet rate threshold that keeps \pninty latency below the target latency at a \textit{normal core}\\
    \hline
    $CR$ & Real[$C$] & The aggregated packet rate assigned to a \textit{normal core} \\
    \hline
    $CF$ & Integer[$C$] & The total number of flows processed by a \textit{normal core} \\
    \hline
    \end{tabular}
}
% \vspace*{\fill}
\caption{Constants and variables used in \sysname's long-term optimization problem formulation}
\label{t:long-term-parameter}
\end{table}

% what is the key idea behind the algorithm
\parab{Detailed algorithm.} The core of \sysname's long-term scaling is solving an optimization problem: for each worker, to pack a fixed number of RSS buckets into \textit{the least number of normal cores} while avoiding \textit{any persistent overloads}.
In \sysname, a persistent overload is a traffic change that builds up a packet queue that exceeds \sysname's short-term optimization's processing ability.
Given a NF chain's performance profile, this problem can be reduced to a standard bin-packing problem, which is proved to be an NP-Hard problem.

Therefore, in \sysname, we model the problem as a constrained Mixed Integer Linear Programming (MILP) problem. The problem formulation is described as follows:

% This approach is on the other end of the spectrum, trading off speed for a more optimal solution.

\begin{align}
%\min & \qquad P_{r}[T_{c}[i]] - T_{r}[i] & \label{long_obj} \\
\min & \qquad \sum_{i = 1}^{C} CPU_{i} & \label{long_obj} \\
s.t. & \sum_{i = 1}^{C} M_{i,j} = 1 & \forall j, 0 < j < F \label{long_eq1} \\
& CR_i = \sum_{j = 1}^{F} M_{i,j} * BR_j &  \forall i, 0 < i < C \label{long_eq2} \\
& CF_i = \sum_{j = 1}^{F} M_{i,j} * BF_j & \forall i, 0 < i < C \label{long_eq3} \\
& T[CF_i] \geq CR_i& \forall i, 0 < i < C \label{long_eq4} \\
& CPU_i * F - \sum_{j = 1}^{F} M_{i,j} \geq 0 & \forall i, 0 < i < C \label{long_eq5}
\end{align}




\tabref{t:long-term-parameter} lists all constants and variables used in the optimization problem formulation.

$F$ and $C$ are the number of RSS buckets and normal CPU cores in a \sysname worker. $BR$ and $BF$ are arrays of size $F$: they are system measurements that record the packet rate and the number of active flows for each bucket.
$T$ is the offline NF chain's performance profile.
Given a certain number of active flows, it gives a packet rate threshold that keeps the chain's \pninty latency below the optimization's target tail latency SLO. The logic is that \sysname's long-term optimization works for most packets that are not part of transient bursts; on top of that, \sysname's short-term optimizations scales out in smaller traffic and time scales to control the per-packet latency for the rest of traffic. Together, they can achieve microsecond-scale tail latency SLOs.
$CR$ and $CF$ are calculated parameters: they are the aggregated packet rate and total number of flows assigned to a \sysname's normal core.

$M$ is the algorithm's output, which specifies the bucket-to-core assignment produced by the long-term optimization.


We then explain the optimization's objective and constraints: the objective is to minimize the number of active normal CPU cores (\eqnref{long_obj}). \eqnref{long_eq1} ensures that each RSS bucket is assigned to only 1 core. \eqnref{long_eq2} calculates the total flow rate at each normal core and assigns it to an intermediate variable. \eqnref{long_eq3} does the same thing for flow counts. \eqnref{long_eq4} restricts the aggregated packet rate at any normal core from exceeding the packet rate threshold, given the NF chain's performance profile. \eqnref{long_eq5} defines an active core to be a core with at least one assigned RSS bucket.
The idea of this model is that \sysname can achieve a compact load packing when the aggregated packet rate at any normal core is close to but not exceeding the packet rate threshold that corresponds to the target latency.


We also come up with a heuristic that uses the idea of \textit{lazy migration}. The heuristic considers both the number of normal cores and the number of bucket migrations. It works in two steps. \textit{Handling persistent overloads}: it first checks the set of active normal cores, finds normal cores with excessive traffic loads, and determines the set of RSS buckets to be migrated; then, it tries to re-assign these RSS buckets to existing normal cores, following the first-fit policy; if all current active normal cores are full, the algorithm brings up one additional normal core. It iterates until all buckets are assigned to a normal core. Second, \textit{re-packing}: the algorithm finds the core with the lowest aggregated packet rate, and tentatively assigns its buckets to other cores. If it succeeds, the core is reclaimed from the system. All buckets previously associated with the core are migrated accordingly.
The heuristic then repeats the re-packing process until no cores can be reclaimed.

% Now, we know that our current system does not handle a persistent load change properly, so that a persistent load change will (1) create a large software queue at a normal core; (2) increase the short-term optimization overhead because it involves scanning the software queue, which further increases the pipeline’s overhead and exacerbate the problem of a persistent load change.


\parab{On-demand optimization.}
Persistent load changes can happen in between two consecutive long-term optimizations, because of significantly increased packet rates of existing flows and an increased flow arrival rate.
In such cases, one normal core may observe a large software queue, which then requires \sysname's short-term optimization to migrate a subset of flows from the queue.
However, the short-term optimization can introduce large overheads when many packets present in a software queue, as the short-term optimization expects rare bursts in traffic and assumes small software queues, and fails to absorb the large queue effectively within a small number of short-term epochs.
Therefore, when a normal core observes a large queue (e.g., 256 packets in a normal core's software queue), it will trigger a \sysname's long-term optimization immediately\footnote{\sysname has to respect the hardware limitation of modifying rules at the NIC's flow table. At each server, we set a lower bound on the time interval of two long-term optimizations as 5 milliseconds (for Mellanox ConnectX-5 100 GbE).} to split its traffic into two subsets. One subset is marked to be migrated by the above two-step heuristics. After that, the current long-term epoch is reset.






==> op_short.tex <==

\subsection{Absorbing bursts with short-term optimizations}
\label{subsec:short-term-op}

The procedure of absorbing transient bursts at a normal core is called the \textit{short-term optimization}.
This optimization is executed recurrently at every normal core.
This is to make sure that a normal core is able to detect a burst at its designated queue and also have enough time to process the burst with the help of nearby computing resources, i.e. sidecar cores on the same server.

% explain how the system absorbs transient bursts
\parab{Flows, software queues and sidecar cores.} Each normal CPU core is associated with one NIC queue. \sysname's ingress allocates traffic aggregates to each queue. Ideally, \sysname's ingress should ensure that each normal core is able to process its assigned traffic without latency SLO violations.
However, this can lead to over-provisioning of normal cores because most bursts are transient rather than persistent, and can happen between two consecutive scaling events.

Without over-provisioning cores statically to prepare for transient bursts, \sysname allows transient bursts to happen at normal cores, and utilizes the periodical short-term optimization to to borrow nearby system resources needed to process excessive traffic that may cause SLO violations.

\parab{Detecting transient bursts.} A transient burst happens when excessive traffic arrives at a NIC queue that cannot be handled by one normal core without any latency SLO violations. For each NF chain, the normal core relies on an offline performance profile to determine whether the existing NIC backlog queue needs extra computing resources to avoid SLO violations. Under a certain number of active flows, the performance profile gives the maximum number of packets that can be processed by $N$ CPU cores, where $N$ can be a number of cores on which an NF chain can run.



\begin{figure}[tb!]
\resizebox{0.95\columnwidth}{!}{
    \includegraphics[width=\textwidth]{figs/normal_core.pdf}
}
\caption{The short-term optimization pipeline executed recurrently at each normal core. It maintains per-epoch packet and flow counters to track packets and flows being queued at the core. Once a large backlog queue is detected, the short-term optimization reacts by splitting the queue into multiple software queues, and requesting a corresponding number of sidecar cores to process them.}
\label{fig:short-term-pipeline}
\end{figure}



\figref{fig:short-term-pipeline} shows the design of a normal core's pipeline for detecting transient bursts and borrowing reserved cores on the same server to help absorb them.



% short-term epoch = 0.5 target SLO
\parab{Detailed algorithms .}
At each normal core, packet scheduling happens in \textit{short-term epochs}.
\sysname determines the period of short-term optimizations to be \textit{half of the target tail latency SLO}.
For example, if the target tail latency SLO is 200 $\mu$s, each normal core's pipeline should gather traffic statistics and execute the short-term optimization every 100 $\mu$s.
The optimization procedure is executed at the end of a short-term epoch, and aims to borrow just-enough stand-by computing resources (i.e. reserved CPU cores on the same server) to absorb a backlog packet queue at the designated NIC queue by the end of the next epoch.
The intuition is that: suppose \sysname's short-term optimization is able to process all packets in the existing packet queue at the beginning of a short-term epoch; then, at any normal core, a packet will be queued for at most 2 consecutive short-term epochs, which exactly matches the target tail latency SLO.

As \sysname targets microsecond-scale latency SLOs, this short-term optimization period (or the duration of a short-term epoch) is also at microsecond-scale, and is 1000-10000 times smaller than other NFV systems' auto-scaling or load balancing time granularity ~\cite{conext19-rsspp,wang2021galleon,infocom22-dyssect}).
This difference in the algorithm's time granularity is the key for meeting microsecond-scale tail latency SLOs.

% \KwData{$core_{id}$ (normal core's unique ID)}
% \KwData{$q_{local}$ (normal core's own software queue)}
% \KwData{$q_{sw}$ (a vector of standby software queues)}
% \KwData{$f_{active}$ (a vector of active flows)}
% \Comment{Update traffic stats for software queues}
% \For{$q\gets $ \  $q_{sw}.begin()$ \KwTo $q_{sw}.end()$}{
%     $q.pkts\_queued = q.pkts\_arrival - q.pkts\_processed$
% }

% the algorithm box
\algnewcommand{\LeftComment}[1]{\State \(\triangleright\) #1}
\newcommand{\pluseq}{\mathrel{+}=}

\begin{algorithm}[tb]
\caption{Updating the number of queued packets and flows at a normal core at the end of a short-term epoch}\label{alg:short_term_op1}
\begin{algorithmic}[1]
\Statex \textbf{Input:}
%Q$_{local}$ \textit{(the default software queue used by this core)}
\Statex ActiveFlows: \textit{a vector of flows w/ packet arrivals in the last epoch. Sorted based on the queued packet count in ascending order}
\Statex Queues: \textit{a vector of software queues currently owned by this normal core. Queues[0] is its local queue.}
\Statex FlowToQueueMap: \textit{a map that records its target software queue for a flow}
% \Statex
\Procedure{UpdateStatsForPastEpoch}{}
\LeftComment{\textcolor{blue}{Update traffic statistics for all software queues}}
\For{\textbf{all} $q$ $\in$ Queues}
    \State $q.pkts.queued \gets$\par
     \hskip\algorithmicindent $q.pkts.arrival - q.pkts.processed$
    \State $q.flows.queued \gets 0$ \Comment{\textcolor{blue}{To be updated below}}
\EndFor

\LeftComment{\textcolor{blue}{Update task sizes for active flows}}
\For{\textbf{all} $f$ $\in$ ActiveFlows}
    \State $f.pkts.queued \gets$\par
     \hskip\algorithmicindent $f.pkts.arrival - f.pkts.processed$
    \State $f.task\_size \gets f.pkts.queued$
    \LeftComment{\textcolor{blue}{Update flow count for $f$'s associated $q$}}
    \State $q \gets$ FlowToQueueMap[$f$]
    \State $q.flows.queued \pluseq 1$
\EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}



Here, we explain the short-term optimization step by step.
First, the normal core updates per-software-queue traffic statistics as shown in \algoref{alg:short_term_op1}. Traffic statistics includes the number of packets that have arrived and processed, and the number of flows that have arrived and processed in the past epoch.
Note: an active flow is defined as a flow that has any packet arrivals in the past epoch.

% At NFVCore:
% Step
% 0 (last epoch ends, epoch start)
% If |epoch_packet_arrival_| > |epoch_packet_processed|, then a packet queue exists.

% 1 Update |unoffloaded_flows_|;  // each w/ its # of packets in NIC queue

% 2 Update |sw_q_| to see the packet room for each queue; f(active flow count, packet count)

% 3 Greedily assign flows in |unoffloaded_flows_| to the normal core’s software queue, and then existing (borrowed) software queues; If more queues are needed, call RequestNQ() to get more from NFVCtrl;

% 4 Check all (borrowed) software queues to find overloaded ones.
% If found, then migrates flows from the queue to other software queues.
% If more queues are needed, call RequestNQ() to get more from NFVCtrl;

% 5 Assign remaining flows (they are rare busty flows) to standalone software queues, and decide to split an NF chain into multiple cores;
% Note:
% the splitting depends on the NF profiling and targets the smallest number of cores;
% If the system cannot handle a flow anyway, then we can’t do anything about it;

% 6 Return software queues if they have been idle for N short epochs;

\begin{algorithm}[tb!]
\caption{Absorbing transient bursts at a normal core at the end of a short-term epoch}\label{alg:short_term_op2}
\begin{algorithmic}[1]
\Statex \textbf{Input:}
\Statex CoreID: \textit{The normal core's unique ID}
\Statex MaxSplit: \textit{The max number of cores in which the target NF chain can be split}
\Statex Profile: \textit{The short-term performance profile which tells the max packet rate given the execution scheme (1st arg: \# of cores) and  traffic (2nd arg: flow count).}
% \Statex
\LeftComment{Given a software queue Q, check and migrate excessive flows to other queues}
\Procedure{HandleSoftwareQueue}{Queue Q}
    \State SumTask $\gets 0$
    \State UnoffloadedF $\gets \{\}$
    \State AlertF $\gets \{\}$
    \LeftComment{\textcolor{blue}{Collects all flows destined to Q}}
    \For{\textbf{all} $f$ $\in$ ActiveFlows}
        \If{$f.target\_q$ is Q} THEN
            \LeftComment{\textcolor{blue}{Check if $f$ fits in Q w/ 1 core processing}}
            \If{SumTask$+ f.task\_size \leq$\par
            \hskip\algorithmicindent Profile(1, UnoffloadedF.Size()$+ 1$)}
                \State UnoffloadedF.Add($f$)
                \State SumTask $\pluseq f.task\_size$
            \Else
                \If{MigrateFlowToQueue($f$)}
                    \State continue \Comment{$f$ has been migrated}
                \EndIf
                \LeftComment{\textcolor{blue}{Fail to process $f$ w/o SLO violations}}
                \State AlertF.Add($f$)
            \EndIf
        \EndIf
    \EndFor
    \LeftComment{\textcolor{blue}{Notify whale flows with large instantaneous rates}}
    \State RaiseAlert(CoreID, AlertF)
\EndProcedure
\State
\LeftComment{Migrate one flow under the first-fit policy. Return true if it succeeds, otherwise false}
\Procedure{MigrateFlowToQueue}{Flow F}
    \For{\textbf{all} $q$ $\in$ Queues}
        \For{$core\_num$ $\gets q.split$ to MaxSplit}
            \If{$q.pkts.queued + $ F$.task\_size \leq$\par
            Profile($core\_num$, $q.flows.queued + 1$)}
                \State FlowToQueueMap[F] = q
                \State $q.split$ = $core\_num$
                \State \Return True
            \EndIf
        \EndFor
    \EndFor
    \State \Return False
\EndProcedure
\end{algorithmic}
\end{algorithm}


Then, it goes through all software queues, including the local queue and other queues, shown in \algoref{alg:short_term_op2}.
This is to determine whether a software queue owns excessive traffic that cannot be handled by one CPU core.
Next, it goes through all active flows, and maintains a set of flows (called \textit{unoffloaded flows}) that are present in the local software queue.
It iterates through \textit{unoffloaded flows} to determine whether these flows can be handled by one core. If not, flows need to be migrated from the local software queue to another software queue so that they can be processed by sidecar cores on the same server.

The flow re-assignment includes two parts: the normal core first tries to fit flows greedily in its local software queue to minimize the number of migrated flows. The core then applies the first-fit policy to allocate excessive flows to other queues.

In some cases, there are whale flows with large instantaneous packet rates.
These flows can have a significant large number of packets in a software queue.
At the end of a short-term epoch, \sysname's short-term optimization algorithm may find that: for a single flow, the number of queued packets can even exceed a single core's processing capability in the new short-term epoch.
It may still lead to latency SLO violations if \sysname simply migrates these flows to software queues and assigns each queue a sidecar core. 

For these cases, \sysname introduces an NF chain splitting mechanism that splits an NF chain into multiple sub-chains. Each sub-chain runs by a unique sidecar core.
Together, sub-chains form a complete chain and process packets in a pipeline, which accelerates the NF chain to increase the max number of packets that can be processed within a short-term epoch.
For each whale flow, \sysname moves them to one dedicated software queue, and selects a number of sidecar cores to run the split NF chain.
Splitting a chain into multiple cores can downgrade the average per-core performance.
Therefore, \sysname determines the NF-chain splitting by choosing the number of sidecar cores as the minimal number of cores required to process queued packets of a whale flow in the next short-term epoch.

We acknowledge that even with NF-chain splitting, \sysname can still be limited by the upper-bound of the number of packets that can be processed in a short epoch.
For a significantly bursty flow, \sysname may find it impossible to process it without latency SLO violations.
Thus, \sysname moves the flow to a dedicated software queue, processes its queued packets, and allows SLO violations.
In the meantime, \sysname produces a system warning that reports this problematic flow.


